Inferring Super-Resolution Depth from a Moving Light-Source Enhanced RGB-D Sensor: A Variational Approach

A novel approach towards depth map super-resolution using multi-view uncalibrated photometric stereo is presented. Practically, an LED light source is attached to a commodity RGB-D sensor and is used to capture objects from multiple viewpoints with unknown motion. This non-static camera-to-object setup is described with a nonconvex variational approach such that no calibration on lighting or camera motion is required due to the formulation of an end-to-end joint optimization problem. Solving the proposed variational model results in high resolution depth, reflectance and camera pose estimates, as we show on challenging synthetic and real-world datasets.

==> figures/realworld_qualitative.tex <==
%\begin{figure}[!ht]
%  \centering
%  \setlength\tabcolsep{1pt} % horizontal spacing between columns. Default: 6pt
%  \def\arraystretch{0} % vertical spacing between rows. Default: 1
%  \newcommand{\mywidth}{0.11\textwidth} % for max width on {one,two} column(s) assume total page width to be {0.86,0.97}.
%  \newcommand{\mywidthlr}{0.08\textwidth} % for max width on {one,two} column(s) assume total page width to be {0.86,0.97}.
%
%  \newcolumntype{C}{>{\centering\arraybackslash}m{0.02\textwidth} }
%  \newcolumntype{X}{>{\centering\arraybackslash}m{\mywidth}}
%  \newcolumntype{Y}{>{\centering\arraybackslash}m{\mywidthlr}}
%  \begin{tabular}{CXYXX}
%    \rotatebox{90}{Coat}&
%    \includegraphics[width=\mywidth]{realworld/coat2}&
%    \includegraphics[width=\mywidthlr]{realworld/coat_D}&
%    \includegraphics[width=\mywidth]{realworld/coat_r}&
%    \includegraphics[width=\mywidth]{realworld/coat_N_refine}\\
%    \rotatebox{90}{Hat}&
%    \includegraphics[width=\mywidth]{realworld/hat3}&
%    \includegraphics[width=\mywidthlr]{realworld/hat_D}&
%    \includegraphics[width=\mywidth]{realworld/hat_r}&
%    \includegraphics[width=\mywidth]{realworld/hat_N_refine}\\
%    \rotatebox{90}{Cap}&
%    \includegraphics[width=\mywidth]{realworld/cap}&
%    \includegraphics[width=\mywidthlr]{realworld/cap_D}&
%    \includegraphics[width=\mywidth]{realworld/cap_z}&
%    \includegraphics[width=\mywidth]{realworld/cap_N}\\
%    \rotatebox{90}{Pillow}&
%    \includegraphics[width=\mywidth]{realworld/pollow}&
%    \includegraphics[width=\mywidthlr]{realworld/pollow_D}&
%    \includegraphics[width=\mywidth]{realworld/pollow_z}&
%    \includegraphics[width=\mywidth]{realworld/pollow_N}\\
%    &$I_{ref}$& Input Depth & Refined Depth & Refined Normals
%  \end{tabular}
%  \caption{Results of our approach on challenging real-world datasets.}
%  \label{fig:realworld_qualitative}
%\end{figure}

\begin{figure}[!ht]
  \centering
  \setlength\tabcolsep{1pt} % horizontal spacing between columns. Default: 6pt
  \def\arraystretch{0} % vertical spacing between rows. Default: 1
  \newcommand{\mywidth}{0.18\textwidth} % for max width on {one,two} column(s) assume total page width to be {0.86,0.97}.
  \newcommand{\mywidthlr}{0.11\textwidth} % for max width on {one,two} column(s) assume total page width to be {0.86,0.97}.

  \newcolumntype{C}{>{\centering\arraybackslash}m{0.02\textwidth} }
  \newcolumntype{X}{>{\centering\arraybackslash}m{\mywidth}}
  \newcolumntype{Y}{>{\centering\arraybackslash}m{\mywidthlr}}
  \begin{tabular}{XX}    
    \includegraphics[width=\mywidth]{realworld/jacket_patch_rgb}&
    \includegraphics[width=\mywidthlr]{realworld/jacket_patch_input} \\
    RGB image & input depth map  \\
   
    \includegraphics[width=\mywidth]{realworld/jacket_patch_color}&
    \includegraphics[width=\mywidth]{realworld/jacket_patch} \\
    
  3D model & refined depth
  \end{tabular}
  \caption{Results of our approach on challenging real-world datasets.}
  \label{fig:realworld_qualitative}
\end{figure}


==> figures/synthetic_bunny.tex <==
\begin{figure}[!ht]
  \centering
  \setlength\tabcolsep{0pt} % horizontal spacing between columns. Default: 6pt
  \def\arraystretch{0.5} % vertical spacing between rows. Default: 1
  \newcommand{\mywidth}{0.115\textwidth} % for max width on {one,two} column(s) assume total page width to be {0.86,0.97}.
  \newcommand{\mywidthlr}{0.08\textwidth} % for max width on {one,two} column(s) assume total page width to be {0.86,0.97}.

  \newcolumntype{X}{>{\centering\arraybackslash}m{\mywidth}}
  \begin{tabular}{XXXX}
    \includegraphics[height=\mywidth]{synthetic/bunny_13}&
    \includegraphics[height=\mywidth]{synthetic/bunny_13_rho}&
    \includegraphics[height=\mywidthlr]{synthetic/bunny_13_D}&
    \includegraphics[height=\mywidth]{synthetic/bunny_13_depth_refine}\\
    RGB Image & Estimaged Albedo & Input Depth & Refined Depth\\
    \includegraphics[height=\mywidthlr]{synthetic/bunny_13_N_raw}&
    \includegraphics[height=\mywidthlr]{synthetic/err}&
    \includegraphics[height=\mywidth]{synthetic/bunny_13_N}&
    \includegraphics[height=\mywidth]{synthetic/err_refine}\\
    Initial Normals & Normal Error & Estimated Normals & Normal Error
  \end{tabular}
  \caption{The input RGB and depth image of reference frame with resolution $960\times1280$ and $480\times640$ and the input normals has MAE $72.9405$ . As a results, refined albedo has RMSE $0.1178$, the refined depth has RMSE $0.0306$ and the refined normals has MAE $16.1252$.}
  \label{fig:synthetic_bunny}
\end{figure}



==> figures/synthetic_joy.tex <==
\begin{figure}[!ht]
  \centering
  \setlength\tabcolsep{0pt} % horizontal spacing between columns. Default: 6pt
  \def\arraystretch{0.5} % vertical spacing between rows. Default: 1
  \newcommand{\mywidth}{0.115\textwidth} % for max width on {one,two} column(s) assume total page width to be {0.86,0.97}.
  \newcommand{\mywidthlr}{0.08\textwidth} % for max width on {one,two} column(s) assume total page width to be {0.86,0.97}.

  \newcolumntype{X}{>{\centering\arraybackslash}m{\mywidth}}
  \begin{tabular}{XXXX}
    \includegraphics[height=\mywidth]{synthetic/joy1}&
    \includegraphics[height=\mywidth]{synthetic/joy1_rho}&
    \includegraphics[height=\mywidthlr]{synthetic/joy_1_D}&
    \includegraphics[height=\mywidth]{synthetic/joy_1_refine}\\
    RGB Image & Estimaged Albedo & Input Depth & Refined Depth\\
    \includegraphics[height=\mywidthlr]{synthetic/joy_N}&
    \includegraphics[height=\mywidthlr]{synthetic/joy_err}&
    \includegraphics[height=\mywidth]{synthetic/joy_N_refine}&
    \includegraphics[height=\mywidth]{synthetic/joy_err_refine}\\
    Initial Normals & Normal Error & Estimated Normals & Normal Error
  \end{tabular}
  
  \caption{The input RGB and depth image of reference frame of resolution $960\times1280$ and $480\times640$ respectively, and the initial normals (MAE $=73.2175$). The refined depth has resolution $960\times1280$ (RMSE $0.0465$) and the refined normals with MAE $12.5415$.}
  \label{fig:synthetic_joy}
\end{figure}


